BAMAX: Backtrack Assisted Multi-Agent Exploration using Reinforcement Learning

Autonomous robots collaboratively exploring an unknown environment is still an open problem. The problem has its roots in coordination among non-stationary agents, each with only a partial view of information. The problem is compounded when the multiple robots must completely explore the environment. In this paper, we introduce Backtrack Assisted Multi-Agent Exploration using Reinforcement Learning (BAMAX), a method for collaborative exploration in multi-agent systems which attempts to explore an entire virtual environment. As in the name, BAMAX leverages backtrack assistance to enhance the performance of agents in exploration tasks. To evaluate BAMAX against traditional approaches, we present the results of experiments conducted across multiple hexagonal shaped grids sizes, ranging from 10x10 to 60x60. The results demonstrate that BAMAX outperforms other methods in terms of faster coverage and less backtracking across these environments.

==> content/traditional_methods.tex <==
In our maze exploration efforts, we have utilized different conventional approaches such as Depth First Search (DFS), Breadth First Search (BFS),Collaborative DFS and Collaborative BFS.

\subsection{DFS(Depth First Search):}
In a hexagonal grid, the Depth First Search (DFS) algorithm starts from a given starting node and proceeds by exploring as far as possible along each branch before backtracking. This means that DFS tends to follow a zig-zag pattern through the grid, delving deeply into one branch before backtracking and exploring a different branch. The advantage of DFS in this context is its ability to quickly explore and traverse deep into the grid.

\subsection{BFS(Breadth First Search):}
BFS, on the other hand, involves starting from the starting node and exploring all nodes at the current depth level before moving on to the next depth level. This means that BFS will explore the grid in a more systematic manner, covering all nodes at the same depth level before moving on to the next depth level.

In DFS and BFS we are not sharing the grid map between multiple agents. This can causes the problem of multiple agents revisiting cells in DFS and BFS, to address this problem, we have made enhancements known as Collaborative DFS and Collaborative BFS. These modified algorithms aim to improve the efficiency of exploring the entire grid by facilitating the sharing of the grid map among multiple agents. By preventing cell revisits, the collaborative versions help reduce the overall exploration time required.

\subsection{Collaborative DFS:}
\cite{MAKKI19967}

In Collaborative DFS, the grid map is shared among multiple agents, ensuring that no cell is revisited by any agent. This sharing is facilitated through the use of data structures, such as graphs, which track the visited and unvisited cells and are accessible to all agents. When an agent reaches the end of a branch, it seeks the nearest unvisited cell from its current position (calculated using eq: \ref{eq:distance-between-cells}) and navigates there using the A* algorithm \cite{4082128}. It is possible for the nearest cell to be from another agent's exploration branch that has not yet been visited.

\begin{equation}
  \text{distance}(cell1, cell2) = \sqrt{{(x_2 - x_1)}^2 + {(y_2 - y_1)}^2}
  \label{eq:distance-between-cells}
\end{equation}

where $(x_1, y_1)$ and $(x_2, y_2)$ are the coordinates of the two cells. \\

\begin{algorithm}[H]
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}

  \Input{$graph$, $N$ agents}
  
  \For{agent $n$ in $N$ agents}{
    \If{environment not fully explored}{
      Update the graph with $a_{n}^N$ current position\;
      
      \If{agent reaches end of a branch}{
        $nearest\_cell$ = get nearest unvisited cell from current cell using a distance metric\;
        $all\_cells\_distance$ = []\;
        
        \For{cell in unvisited cells}{
          Calculate distance between agent's current cell and cell\;
          Update $all\_cells\_distance$ with calculated distance\;
        }
        
        $nearest\_cell$ = minimum distance from $all\_cells\_distance$\;
        Get path to $nearest\_cell$ using $A*$ algorithm\;
        
        \For{cell in $nearest\_cell\_path$}{
          $next\_unexplored\_cell$ = cell\;
        }
      }
      \Else{
        $next\_unexplored\_cell$ = get next cell from current branch\;
      }
      
      $agent\_with\_next\_unexplored\_cell$ = $next\_unexplored\_cell$\;
      \Return $agent\_with\_next\_unexplored\_cell$\;
    }
  }
  
  \caption{Collaborative DFS}
\end{algorithm}



\begin{table}
\centering
\caption{Comparison of DFS, BFS with collaborative DFS, BFS}\label{tab1}
\begin{tabular}{|p{4cm}|l|l|}
\hline
\textbf{Method Name} &  \textbf{Grid Size} & \textbf{Average Steps taken to explore}\\
\hline
DFS & {10x10} & 149\\
BFS & {10x10} & 339\\
Collaborative DFS & {10x10} & 59\\
Collaborative BFS & {10x10} & 230\\
\hline
\end{tabular}
\end{table}
